Non-idempotent types for classical calculi in natural deduction style

In the first part of this paper, we define two resource aware typing systems for the {\lambda}{\mu}-calculus based on non-idempotent intersection and union types. The non-idempotent approach provides very simple combinatorial arguments-based on decreasing measures of type derivations-to characterize head and strongly normalizing terms. Moreover, typability provides upper bounds for the lengths of the head reduction and the maximal reduction sequences to normal-form. In the second part of this paper, the {\lambda}{\mu}-calculus is refined to a small-step calculus called {\lambda}{\mu}s, which is inspired by the substitution at a distance paradigm. The {\lambda}{\mu}s-calculus turns out to be compatible with a natural extensionof the non-idempotent interpretations of {\lambda}{\mu}, i.e., {\lambda}{\mu}s-reduction preserves and decreases typing derivations in an extended appropriate typing system. We thus derive a simple arithmetical characterization of strongly {\lambda}{\mu}s-normalizing terms by means of typing.

==> alternative.tex <==
\section{Alternative}


\begin{itemize}
\item  If  $t_1 , \ldots  , t_n\ (n \geq 0) \in \ISN{\lmu}$, then $x\,t_1 \ldots t_n \in \ISN{\lmu}$. 
\item If  $t \in \ISN{\lmu}$, then $\l x.t \in \ISN{\lmu}$. 
\item If  $\Com  \in \ISN{\lmu}$, then $\mu \al.\Com \in \ISN{\lmu}$. 
\item If  $t \in \ISN{\lmu}$, then $\co{\al}t \in \ISN{\lmu}$.
\item If $u, t\isubs{x/u}\vec{v}\ (n \geq 0) \in \ISN{\lmu}$, then $(\l x.t)u \vec{v} \in \ISN{\lmu}$. 
\item If $u, (\mu \al. \Com\ire{\al}{u})  \vec{v}\ (n \geq0)  \in \ISN{\lmu}$, then $(\mu \al.\Com)u \vec{v}\in \ISN{\lmu}$. 
\end{itemize}

For any $\lmu$-object $o$, we write $\mrl{o}$ for the length of the maximal reduction sequence starting at $o$ ($\mrl{o}<\infty$ iff $o\in \SN{\lmu}$). We have the following equations


\[ \begin{array}{llll}
  \mrl{x\,t_1 \ldots t_n} & = & +_{i=1 \ldots n} \mrl{t_i}\\
  \mrl{\l x.t } & = & \mrl{t}\\
  \mrl{\mu \al.\Com} & = &  \mrl{\Com}\\
  \mrl{\co{\al}t } & = & \mrl{t}\\
  \mrl{(\l x.t)u\, \vec{v}} & = & \mrl{t\isubs{x/u}\vec{v}} + 1 & \mbox{ if }  x \in \fv{t}\\
  \mrl{(\l x.t)u\, \vec{v}} & = & \mrl{u} + \mrl{t\vec{v}} + 1 & \mbox{ if }  x \notin \fv{t}\\
  \mrl{(\mu \al.\Com)u \vec{v} } & = & \mrl{(\mu \al. \Com\ire{\al}{u})\vec{v}} + 1 & \mbox{ if }  \al  \in \fv{\Com}\\
  \mrl{(\mu \al.\Com)u \vec{v} } & = &  \mrl{u} + \mrl{(\mu \al. \Com)\vec{v}} +
 1 & \mbox{ if }  \al  \notin \fv{\Com}\\
  \end{array} \]


\begin{lem} 
\label{l:typable-isn}
If  $o$ is $\Slmu$-typable, \ie\ $\Phi \tri\Gam \vdash o:\Any \mid \Del$, then  $o  \in  \SN{\lmu}$. Moreover,
$\mrl{o} \leq \sz{\Phi}$. 
\end{lem}


\begin{proof} We show $o \in \SN{\lmu} = \ISN{\lmu}$
  and $\mrl{o} \leq \sz{\Phi}$
  by induction on $\sz{\Phi}$, where $\Phi \tri\Gam \vdash o:\Any \mid
  \Del$.  When $\Phi$ does not end with the rule $(\app)$ the proof
  holds straightforwardly by the \ih\ so we consider that $\Phi$ ends
  with $(\app)$, where $\Any = \UM$ and $o = x\,t_1 \ldots t_n$ or $o =
  (\mu \al. \Com)t_1 \ldots t_n$ or $o = (\l x.  u)t_1 \ldots t_n$,
  with  $n \geq 1$. \\

In all the three cases for $o$, there are subderivations
$(\Phi_{i})_{i \in \cset{1 \ldots n}}$ such that $\sz{\Phi_{i}} <
\sz{\Phi}$ so that the \ih\ gives $t_i \in \SN{\lmu} = \ISN{\lmu}$ and
$\mrl{t_i} \leq \sz{\Phi_{i}}$. Now, there are three different cases
to consider: \\

\begin{itemize}
\item[(1)]
 If $o=x\,t_1 \ldots t_n$, then there are \delia{non-empty} subderivations $\Phi_1\ldots \Phi_n$ of $\Phi$ typing $t_1\ldots t_n$ respectively. Since $+_{i=1\ldots n} \sz{\Phi_i} + n+1 \leq \sz{\Phi}$, the \ih\ gives $t_i\in \ISN{\lmu}$  and $\mrl{t_i}\leq \sz{\Phi_i}$ for $1\leq i \leq n$. We conclude since $ \mrl{x\,t_1 \ldots t_n}  =  +_{i=1 \ldots n} \mrl{t_i}$ \\  
  
\item[(2)] If $o = (\mu \al. \Com)t_1 \ldots t_n$, there are two cases: 
\begin{itemize}
 \item $\al \in \fn{\Com}$.  Using  Property~\ref{l:sr}, we get  $\Phi' \tri
   \tyj{(\mu \al. \Com\ire{\al}{t_1}) t_2 \ldots t_n }{\Gam}{\UM \mid
     \Del}$ and $\sz{\Phi'} < \sz{\Phi}$. Then the \ih\ gives $(\mu
   \al. \Com\ire{\al}{t_1}) t_2 \ldots t_n \in \ISN{\lmu}$
   and $\mrl{(\mu \al. \Com\ire{\al}{t_1}) t_2 \ldots t_n } \leq \sz{\Phi'}$. This,
   together with $t_1 \in \ISN{\lmu}$ gives $o  \in
   \ISN{\lmu}$. We conclude since
   $\mrl{o} = \mrl{(\mu \al. \Com\ire{\al}{t_1}) t_2 \ldots t_n } + 1
   \leq   \sz{\Phi'} +1 \leq  \sz{\Phi}$.
   
 \item $\al  \notin \fn{\Com}$. 
Then $\Phi$ is of the form:
   $$
\infer{\infer{
  \infer{\Phi_{\mu\al.\Com}\tri \mu\al.\Com:\umult{\Blind_0}\sep \infer{\Phi_{1}\tri t_1:\VM_1}{\delia{\tri} t_1:\mult{\VM_1}}}{\delia{\tri} (\mu \al.\Com)t_1:\umult{\Blind_1}} }{\delia{\vdots}}\sep \infer{\Phi_{n}\tri t_n:\VM_n}{\delia{\tri} t_n:\mult{\VM_n}}}{\delia{\tri} o:\umult{\Blind_n}}
$$
with \delia{$\UM=\umult{\Blind_n}$}.
\pierre{pour moi, il faut enlever tous les triangles que tu as ajoutes: on ne les mets que sur les feuilles d'arbres (cf. nos preuves d'avant). OK si je les enleve ?}\delia{OK mais est-ce qu'on peut mettre
  par exemple $\ldots \vdash t_2:\mult{\VM_2}$ dans ce cas? le terme tout seule dans l'arbre est bizarre, il faut dire qu'il manque quelque chose}

where  $\mult{\Blind_0}$ is obtained by choice because Lemma~\ref{l:relevance} guarantees that no $\alpha$ is typed in the name assignements of the left derivations. Note that $\sz{\Phi}=+_{i=1\ldots n}\sz{\Phi_i}+\sz{\Phi_{\mu \al.c}}+n$ since \pierre{the} $\Blind_i$ are all blind.
We then build the following derivation:
 $$\Phi_{o'}=\infer{
   \infer{\Phi'_{\mu\al.\Com}\tri \mu\al.\Com:\umult{\Blind_1}\sep \infer{\Phi_{2}\tri t_2:\VM_2}{\tri t_2:\mult{\VM_2}} }{\delia{\vdots}}\sep \infer{\Phi_{n}\tri t_n:\VM_n}{\tri t_n:\mult{\VM_n}}  }
 {\tri o': \umult{\Blind_n}}
 $$
\pierre{pareil pour les triangles} \delia{meme commentaire}
 with $o'=(\mu\al.\Com)t_2\ldots t_n$ and $\Phi'_{\mu\al.\Com}$ the
 derivation $\Phi_{\mu\al.\Com}$ where the choice operator
 raises $\Blind_1$ instead of $\Blind_0$. In particular,
 $\sz{\Phi'_{\mu\al.\Com}}=\sz{\Phi_{\mu\al.\Com}}$, so that
 $\sz{\Phi_{o'}}=+_{i=2\ldots
   n}\sz{\Phi_i}+\sz{\Phi_{\mu\al.\Com}}+n-1< \sz{\Phi}$.
 We also have $\sz{\Phi_1} < \sz{\Phi}$. The \ih\ then gives $o', t_1 \in \ISN{\lmu}$ and $\mrl{o'} \leq \sz{\Phi_{o'}}$ and  $\mrl{t_1} \leq \sz{\Phi_{1}}$. 
 Then in particular $o\in \ISN{\lmu}$. We conclude since:
 $$
\begin{array}[t]{c@{\;}l@{\;}l}
  \mrl{(\mu\al.\Com)t_1\ldots t_n} & = & \mrl{(\mu\al.\Com)t_2\ldots t_n}+\mrl{t_1}+1 \\
  & \leq_{\ih} & \sz{\Phi_{o'}}+\sz{\Phi_{1}}+1\\
  & = &  +_{i=2\ldots n}\sz{\Phi_i}+\sz{\Phi_{\mu\al.\Com}}+n-1 +\sz{\Phi_{1}}+1 \\
  & = & \sz{\Phi}  
\end{array}$$

\pierre{Je me demande si on a vraiment besoin des predicats ISN. Il semble que les egalites sur $\mrl{\_}$ suffisent a conclure} \delia{je suis d'accord mais SN=ISN justifie les equations, il faut quand meme justifier les equations, meme
si on peut dire que c'est straightforward. }
   

 \end{itemize}
\item[(3)] If $o=(\l x. u)t_1 \ldots t_n$, we reason similarly to the
  previous case.
%%  \begin{itemize}
%%  \item $x \in \fv{u}$. 
%%  Using Property~\ref{l:sr} we get $\Phi' \tri  \tyj{u\isubs{x/t_1}t_2 \ldots t_n}{\Gam }{\UM \mid  \Del}$ such that 
%%              $\sz{\Phi'} < \sz{\Phi}$. Then the \ih\ gives 
%%              $u\isubs{x/t_1}t_2 \ldots t_n \in \ISN{\lmu}$. 
%%   This, together with $t_1 \in \ISN{\lmu}$ gives  
%%   $o \in \ISN{\lmu}$.
%% \item $x \notin \fv{u}$.
%%   Then it is easy to build a type derivation
%%   $\Phi'  \tri \tyj{u t_2 \ldots t_n}{\Gam'}{\UM  \mid \Del'}$ verifying
%% $\sz{\Phi'} < \sz{\Phi}$, so that $u t_2 \ldots t_n \in \ISN{\lmu}$ holds by the \ih\ 
%% This, together with with $t_1 \in \ISN{\lmu}$ gives 
%%             $o  \in \ISN{\lmu}$. 
%%  \end{itemize}
\end{itemize}
\end{proof}

\begin{lem} 
  \label{l:isn-typable}
  If $o\in \SN{\lmu}$, then $o$ is $\Slmu$-typable.
\end{lem}

\begin{proof}
  By induction on $\lexnl{o}$. If $o$ is not an application $t\,u$, the inductive step is straightforward. We only detail the case when $o$ is an application.
  \begin{itemize}
  \item If $o = (\mu \al. \Com)t_1 \ldots t_n$, then
    \odelia{$\Any=\UM$ \delia{???} and} we set $o'=(\mu\al.\Com\delia{\ire{\al}{t_1}})t_2\ldots t_n$.
    There are two cases: 
\begin{itemize}
 \item $\al \in \fn{\Com}$. Then $\mrl{o}=\mrl{o'}+1$.  By the \ih\  there is $\Phi_{o'}\tri \muju{\Gam'}{o':\UM}{\Del'}$. By Property~\ref{l:se-s}, there is $\Phi\tri \muju{\Gam'}{o:\UM}{\Del'}$ and we are done.
 \item  $\al \notin \fn{\Com}$. Then $o'=(\mu\al.\Com)t_2\ldots t_n $ and $\mrl{o}=\mrl{o'}+\mrl{t_1}+1$. By the \ih\ there are typing derivations  $\Phi_{o'}\tri \muju{\Gam'}{o':\UM}{\Del'}$ and $\Phi_1\tri \muju{\cdelia{\Gam}{\Gam_1}}{t_1:\VM_1}{\Del_1}$. Since $\al \notin \fn{\Com}$, Lemma~\ref{l:relevance} entails that $\Phi_{o'}$ is of the \delia{following} form, where $\Blind_1$ is a blind type:
    $$
\infer{
  \infer{\Phi'_{\mu\al.\Com}\tri \mu\al.\Com:\umult{\Blind_1}\sep \infer{\Phi_2\tri t_2:\VM_2}{t_2:\mult{\VM_2}}
  }{\delia{\vdots}}\sep \infer{\Phi_{n}\tri t_n:\VM_n}{ t_n:\mult{\VM_n}}}{\muju{\Gam'}{o:\umult{\Blind_n}}{\cdelia{\Del}{\Del'}}}
$$
\end{itemize}
We then set \delia{$\Phi$} as follows:
$$
\infer{
  \infer{\infer{\Phi_{\mu\al.\Com}\tri \mu\al.\Com:\umult{\Blind_0}\sep
\infer{\Phi_1\tri \muju{\Gam_1}{t_1:\VM_1}{\Del_1}}{t_1:\mult{\VM_1}}
    }{
(\mu\al.\Com)t_1:\umult{\Blind_1}
}      \sep \infer{\Phi_2\tri t_2:\VM_2}{t_2:\mult{\VM_2}}
  }{\delia{\vdots}}\sep \infer{\Phi_{n}\tri t_n:\VM_n}{ t_n:\mult{\VM_n}}}{\muju{\Gam'+\Gam_1}{o:\umult{\Blind_n}}{\cdelia{\Del}{\Del'}+\Del_1}}
$$
where $\Phi_{\mu\al.\Com}$ \delia{is exactly as } $\Phi'_{\mu\al.\Com}$ except that we raise the blind type $\Blind_0=\emul \rew \umult{\Blind_1}$ instead of $\Blind_1$.
  \end{itemize}
  
  


\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> macros-answer.tex <==
\long\def\ignore#1{\relax}

\newcommand{\lvec}{\langle}
\newcommand{\rvec}{\rangle}
\newcommand{\lAngle}{\langle\!\langle}
\newcommand{\rAngle}{\rangle\!\rangle}


\newcommand{\contr}[4]{\mathcal{C}_{#1}^{#2|#3}(#4)}
\newcommand{\ren}[3]{\mathcal{R}_{#1}^{#2}(#3)}
\newcommand{\wft}[2]{{#1}\Vdash{#2}}
\newcommand{\colap}[3]{\mathcal{S}_{#1}^{#2}(#3)}

\newcommand{\set}[2]{\mathcal{#1}_{\mathtt{#2}}}
\newcommand{\compF}[2]{\mathtt{#1}\left(#2\right)}
\newcommand{\compFD}[3]{\mathtt{#1}_{\mathtt{#2}}(#3)}
\newcommand{\cmin}[2]{#1\setminus\!\!\!\setminus\, #2}

\newcommand{\quot}[2]{{#1}/\,{#2}}
\newcommand{\minus}[2]{{#1}\backslash {#2}}
\newcommand{\addu}[2]{{#1}\uplus{#2}}
\newcommand{\pos}[1]{\mathtt{pos}(#1)}

\newcommand{\tbul}{\noindent\textbullet~ }
\newcommand{\obj}{o}

%% Types notation
\newcommand{\ty}[2]{{#1} \ftype {#2}}
\newcommand{\ity}[2]{{#1}+{#2}}
%\newcommand{\idity}[2]{{#1}\sqcap {#2}}
%\newcommand{\typ}[2]{\lvec{#1}\vdash{#2}\rvec}
\newcommand{\typ}[2]{\lvec{#1},{#2}\rvec}
\newcommand{\styp}[2]{\lvec{#1}\rhd{#2}\rvec}
%\newcommand{\exptyp}[2]{\lvec{#1}\blacktriangleright{#2}\rvec}
\newcommand{\typs}[3]{\lvec{#1}\vdash_{\scriptscriptstyle #2}{#3}\rvec}
\newcommand{\tyj}[3]{{#2} \vdash #1:#3}
\newcommand{\tyjj}[3]{{#2} \Vdash #1:#3}
\newcommand{\tyjp}[4]{{#2} \vdash_{#4} #1:#3}
\newcommand{\tyjhw}[3]{\tyjp{#1}{#2}{#3}{\headweak}}
\newcommand{\tyjst}[3]{\tyjp{#1}{#2}{#3}{\strong}}
\newcommand{\tyjse}[3]{\tyjp{#1}{#2}{#3}{\stres}}
\newcommand{\tyjva}[3]{\tyjp{#1}{#2}{#3}{\valent}}
%\newcommand{\tyjs}[4]{{#1}\!:\!\lvec{#2}\vdash_{\scriptscriptstyle #3}{#4}\rvec}
\newcommand{\styj}[3]{{#1}\!:\!\lvec{#2}\rhd{#3}\rvec}
\newcommand{\styjs}[4]{{#1}\!:\!\lvec{#2}\rhd_{\scriptscriptstyle     #3}{#4}\rvec}

\newcommand{\tingD}[2]{{#1} \tri {#2}}
\newcommand{\tingE}[2]{{#1} = {#2}}

\newcommand{\subt}[2]{{#1}\leqslant{#2}}
\newcommand{\subtp}[4]{\typ{#1}{#2}\leqslant\typ{#3}{#4}}
\newcommand{\cty}[2]{{#1}\!\Rightarrow\!{#2}}

\newcommand{\rest}{\!\!\downharpoonright}
\newcommand{\srest}{\!\!\upharpoonright}

%\newtheorem{theorem}{{\bf Theorem}}
%\newtheorem{definition}{Definition}
%\newtheorem{example}{Example}
%\newtheorem{lemma}{{\bf Lemma}}[section]
%\newtheorem{corollary}{{\bf Corollary}}
%\newtheorem{property}{{\bf Property}}
%\newtheorem{remark}{{\bf Remark}}

\newtheorem{rmk}{Remark}

\newcommand{\lam}[1]{\lambda #1}
\newcommand{\lx}{\lam{x}}
\newcommand{\dup}[1]{\langle #1 \rangle}
\newcommand{\fv}[1]{\mathtt{fv}(#1)}
\newcommand{\bv}[1]{\mathtt{bv}(#1)}
\newcommand{\fn}[1]{\mathtt{fn}(#1)}
\newcommand{\bn}[1]{\mathtt{bn}(#1)}
\newcommand{\fs}[1]{\mathtt{fs}(#1)}
\newcommand{\bs}[1]{\mathtt{bs}(#1)}
\newcommand{\ol}{\overline{\lambda}}
\newcommand{\nil}{\epsilon}
\newcommand{\vdol}{\vdash_{\ol}}
\newcommand{\vd}{\vdash}
\def\l{\lambda}
\def\Gam{\Gamma}
\def\Sig{\Sigma}
\def\Del{\Delta}
\def\Lam{\Lambda}
\def\Om{\Omega}
\def\sig{\sigma}
\def\del{\delta}
\def\al{\alpha}
\def\gam{\gamma}
\newcommand{\mirule}[2]
   {\renewcommand{\arraystretch}{1.2}
    \begin{tabular}{c} $ #1 $ \\ \hline $ #2 $ \end{tabular}}
\newcommand{\sep}{\hspace*{0.5cm}}
\newcommand{\msep}{\hspace*{0.2cm}}
\newcommand{\Rew}[1]{\rightarrow_{#1}}
\newcommand{\paral}{\Rrightarrow}
\newcommand{\paraln}{\Rrightarrow^*}

\newcommand{\LRew}[1]{\; \! \mbox{}_{#1}{\leftarrow}\ }
\newcommand{\Rewplus}[1]{\rightarrow^{+}_{#1}}
\newcommand{\Rewstar}[1]{\rightarrow^{*}_{#1}}
\newcommand{\Rewn}[2][*]{\rightarrow^{#1}_{#2}}
\newcommand{\SN}[1]{\mathcal{SN}(#1)}
\newcommand{\SNSP}{\mathcal{SN}(\lmu)}
\newcommand{\WN}[1]{\mathcal{WN}(#1)}
\newcommand{\HLN}[1]{\mathcal{L}_{\mathcal{H}}\mathcal{N}(#1)}
\newcommand{\HN}[1]{\mathcal{HN}(#1)}
\newcommand{\HNO}{\mathtt{HO}}
\newcommand{\HNT}{\mathtt{HT}}
\newcommand{\HNCom}{\mathtt{HC}}

\renewcommand{\dot}{;}
\renewcommand{\>}{\rightarrow}
\newcommand{\isubs}[1]{\{ #1 \}}
\newcommand{\irepl}[1]{\{ \! \{  #1 \} \! \}}
\newcommand{\emm}{ [\,] }
\newcommand{\es}{ \emptyset}
\newcommand{\klH}[1]{\lvec #1 \rvec}

\newcommand{\U}{\mathcal{U}}

\newcommand{\V}{\mathcal{V}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\mult}[1]{[#1]}
\newcommand{\umult}[1]{\langle #1 \rangle}
\newcommand{\uumult}[1]{\langle  \! \langle #1 \rangle  \! \rangle}
\newcommand{\cset}[1]{ \{ #1 \} }
\newcommand{\deft}[1]{{\bf #1}}
\newcommand{\ISN}[1]{\mathcal{I}(#1)}
\newcommand{\klop}{\mathtt{K}}
\newcommand{\mklop}{\milner \!    \setminus  \!    \Gc}
\newcommand{\hesklop}{\hes \!    \setminus  \!    \Gc}
\newcommand{\milner}{\mathtt{M}}
\newcommand{\hk}{\mathtt{HK}}
\newcommand{\hmilner}{\hes}
\newcommand{\hes}{\mathtt{E}}
%\newcommand{\hl}{\mathtt{Rea}}
\newcommand{\khes}{\hesklop}

\newcommand{\h}{\mathtt{I}}
\newcommand{\ih}{{\it i.h.}}
\newcommand{\pair}[2]{\langle #1, #2 \rangle}
\def\l{\lambda}
\newcommand{\eps}{\epsilon}
\newcommand{\trid}{\bigtriangledown}

\ignore{
 \newcommand{\cdelia}[2]{\textcolor{blue} {#2}}
 \newcommand{\delia}[1]{\textcolor{blue} {#1}}
 \newcommand{\odelia}[1]{\text{\sout{\delia{#1}}}}

   \newcommand{\cpierre}[2]{\textcolor{red} {#2}}
  \newcommand{\pierre}[1]{\textcolor{red} {#1}}
   \newcommand{\opierre}[1]{\text{\sout{\pierre{#1}}}}
}
\newcommand{\cvinc}[1]{\textcolor{cyan} {#1}}

\newcommand{\acomment}[1]{\textcolor{red} {#1}}
%\newcommand{\acomment}[1]{#1}
\newcommand{\IN}{ ; }
\newcommand{\OUT}{ \ \mathtt{out}\ }

\newcommand{\commands}[1]{\mathcal{C}_{#1}}
\newcommand{\terms}[1]{\mathcal{T}_{#1}}
\newcommand{\contexts}[1]{\mathcal{C}_{#1}}
\newcommand{\objects}[1]{\mathcal{O}_{#1}}
\newcommand{\Objects}{\mathcal{O}}
\newcommand{\lists}[1]{\mathcal{L}_{#1}}
\newcommand{\Lists}{\mathtt{Lists}}
\newcommand{\WTerms}{\Lambda_{\Terms}}
\newcommand{\WObjects}{\Lambda_{\Objects}}
\newcommand{\WLists}{\Lambda_{\Lists}}
\newcommand{\vdhes}{\vdash_{\hes}}
\newcommand{\vdhm}{\vdash_{\hmilner}}
\newcommand{\Unf}[1]{\mathtt{U}(#1)}
\newcommand{\proj}[1]{\mathtt{P}(#1)}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\cf}{{\it cf.}}
\newcommand{\resp}{\textit{resp.}\ }

\newcommand{\eg}{{\it e.g.},\ }
\newcommand{\dist}[1]{ |  \! \! |  #1 | \! \! | }
\newcommand{\maxi} {\mathtt{max}}
\newcommand{\dM}{\l_{\mathtt{lsub}}}
\newcommand{\ccontext}{\mathtt{C}}
\newcommand{\hccontext}{\mathtt{HC}}
\newcommand{\dcontext}{\mathtt{D}}
\newcommand{\hdcontext}{\mathtt{HD}}
\newcommand{\ocontext}{\mathtt{O}}
\newcommand{\hocontext}{\mathtt{HO}}
\newcommand{\pcontext}{\mathtt{P}}
\newcommand{\hpcontext}{\mathtt{HP}}
\newcommand{\ucontext}{\mathtt{U}}
\newcommand{\hucontext}{\mathtt{HU}}
\newcommand{\vcontext}{\mathtt{V}}
\newcommand{\hvcontext}{\mathtt{HV}}


\newcommand{\slist}{\mathtt{L}}
\newcommand{\lheadc}{\mathtt{L}_{\mathtt{H}}}
\newcommand{\headc}{\mathtt{H}}
\newcommand{\mlist}{\mathtt{M}}

\newcommand{\cwc}[1]{{[} \! {[} #1 {]}  \! {]}}
\newcommand{\void}{\_}
\newcommand{\ion}{i=1\ldots n}
\newcommand{\ioz}{i=1\ldots 0}
\newcommand{\iom}{i=1\ldots m}
\newcommand{\ionm}{i=1\ldots n+1}
\newcommand{\jom}{j=1\ldots m}
\newcommand{\jon}{j=1\ldots n}
\newcommand{\kol}{k=1\ldots l}
\newcommand{\izn}{i=0\ldots n}
\newcommand{\op}{\! *}
\newcommand{\size}[1]{\mathtt{tm}(#1)}
\newcommand{\mul}[2]{\mathtt{mul}_{#1}(#2)}
\newcommand{\mX}{X}
\newcommand{\B}{\mathtt{B}}
\newcommand{\Mu}{\mathtt{M}}
\newcommand{\betanil}{\beta_{\nil}}
\newcommand{\betanonnil}{\beta_\mathtt{cons}}

\newcommand{\Bnil}{\mathtt{dB}_{\mathtt{nil}}}
\newcommand{\Cvar}{\mathtt{@}_{\mathtt{var}}}
\newcommand{\Capp}{\mathtt{@}_{\mathtt{app}}}
\newcommand{\Cnil}{\mathtt{C}_{\mathtt{nil}}}
\newcommand{\Ccons}{\mathtt{C}_{\mathtt{cons}}}
\newcommand{\Cassoc}{\mathtt{C}_{\mathtt{assoc}}}
\newcommand{\fix}{\mathtt{B@}}

\newcommand{\Bcons}{\mathtt{dB}_{\mathtt{cons}}}
\newcommand{\Gc}{\mathtt{w}}
\newcommand{\Gcs}{\mathtt{w}_{v}}
\newcommand{\Gcr}{\mathtt{w}_{n}}
\newcommand{\cntr}{\mathtt{c}}
\newcommand{\cntrs}{\mathtt{c}_{v}}
\newcommand{\cntrr}{\mathtt{c}_{n}}
\newcommand{\der}{\mathtt{d}}
\newcommand{\ders}{\mathtt{d}_{v}}
\newcommand{\derr}{\mathtt{d}_{n}}
\newcommand{\sm}{\setminus}
\newcommand{\ssm}{\smallsetminus}
\newcommand{\rrule}[1]{\mapsto_{#1}}
\newcommand{\tri}{\triangleright}
\newcommand{\trip}[1]{\triangleright_{#1}}
\newcommand{\dom}[1]{\mathtt{dom}(#1)}
\newcommand{\myparagraph}[1]{{\normalsize \bf #1}}
\newcommand{\iI}{{i \in I}}
\newcommand{\jJ}{{j \in J}}
\newcommand{\kK}{{k \in K}}
\newcommand{\kL}{{k \in L}}
\newcommand{\lL}{{\ell \in L}}
\newcommand{\Lt}{L_t}
\newcommand{\Lku}{L^k_u}
\newcommand{\Lkv}{L^k_v}

\newcommand{\lLt}{\ell \in \Lt}
\newcommand{\lLku}{\ell \in \Lku}
\newcommand{\lLkv}{\ell \in \Lkv}
\newcommand{\head}{head}
\newcommand{\Head}{Head}
\newcommand{\Weak}{Weak}
\newcommand{\weak}{weak}
\newcommand{\weakly}{weakly}
\newcommand{\linear}{linear}
\newcommand{\Linear}{Linear}
\newcommand{\headweak}{\mathcal{H}\mathcal{W}}
\newcommand{\strong}{\mathcal{Q}}
\newcommand{\stres}{\strong_{\hes}}
\newcommand{\valent}{\mathcal{V}}
\newcommand{\sz}[1]{\compF{sz}{#1}}
\newcommand{\szt}[1]{\compF{sz2}{#1}}
\newcommand{\ax}{\mathtt{ax}}
\newcommand{\cut}{\mathtt{cut}}
\newcommand{\cuthw}{\mathtt{cut}_{\headweak}}
\newcommand{\cuts}{\mathtt{cut}_{\strong}}
\newcommand{\introarrow}{\Rightarrow_{\mathtt{i}}}
\newcommand{\elimarrow}{\Rightarrow_{\mbox{\mathtt{e}}}}
\newcommand{\elimarrowhw}{\Rightarrow{\mbox{\mathtt{e}}}_{\headweak}}
\newcommand{\elimarrows}{\Rightarrow{\mbox{\mathtt{e}}}_{\strong}}
%\newcommand{\arrowright}{\Rightarrow{\mathtt{i}}}
\newcommand{\arrowleft}{\Rightarrow{\mbox{\mathtt{l}}}}
\newcommand{\arrowlefthw}{\Rightarrow{\mbox{\mathtt{l}}}_{\headweak}}
\newcommand{\arrowlefts}{\Rightarrow{\mbox{\mathtt{l}}}_{\strong}}
\newcommand{\simplelist}{\mathtt{hlist}}
\newcommand{\appu}{\Rightarrow_{{\mathtt{e}_1}}}
\newcommand{\appd}{\Rightarrow_{{\mathtt{e}_2}}}
\newcommand{\app}{\Rightarrow_{{\mathtt{e}}}}
\newcommand{\appet}{\Rightarrow_{\mathtt{e}*}}
\newcommand{\appempty}{\Rightarrow_{{\mathtt{empty}}}}
\newcommand{\subs}{\mathtt{s}}
\newcommand{\repl}{\mathtt{r}}

\newcommand{\appin}{\mathtt{app}_{\in}}
\newcommand{\appnotin}{\mathtt{app}_{\notin}}
\newcommand{\appnil}{\mathtt{app}_{nil}}
\newcommand{\concat}{@}
\newcommand{\ES}{\mathtt{es}}
\newcommand{\EShw}{\mathtt{es}_{\headweak}}
\newcommand{\ESs}{\mathtt{es}_{\strong}}
%\newcommand{\lhr}{\mathtt{H}_{\mathtt{L}}}
\newcommand{\lhr}{\mathtt{L}_{\mathtt{H}}}
\newcommand{\mlhr}{\lhr\milner}
\newcommand{\hlhr}{\lhr\hes}
\newcommand{\mhr}{\mathtt{H}\milner}
\newcommand{\hhr}{\mathtt{H}\hes}
\newcommand{\post}[1]{\mathcal{P}(#1)}
\newcommand{\negt}[1]{\mathcal{N}(#1)}
\newcommand{\headmcntr}{\cntr|_{\lhr}}
\newcommand{\headhcntr}{\cntr|_{\lhr}}
\newcommand{\redexocc}[2]{\mathtt{RO}[ \! [ #1 ] \! ](#2)}
\newcommand{\tredexocc}[3]{\mathtt{TRO}[ \! [ #1 ] \! ](#2, #3)}
\newcommand{\Id}{\mathtt{I}}
\renewcommand{\AA}[3]{\mathtt{A}(#1,#2,#3)}
\newcommand{\BB}[3]{\mathtt{B}(#1,#2,#3)}
\newcommand{\subn}{\mathtt{sub}}
\newcommand{\sub}[1]{\subn(#1)}
\newcommand{\et}[1]{(#1)^*}
\newcommand{\down}[1]{(#1)^\downarrow}
\newcommand{\LJT}{LJT}
\renewcommand{\al}{\alpha}
\newcommand{\ga}{\gamma}
\newcommand{\co}[1]{[#1]}
\newcommand{\coal}{\co{\al}}
\newcommand{\ire}[2]{\{ #1 /\! \! /  #2\} }
\newcommand{\bta}{a}
\newcommand{\btb}{b}
\newcommand{\btc}{c}
\newcommand{\sta}{\sig}
\newcommand{\stb}{\rho}
\newcommand{\stc}{\tau}
\newcommand{\M}{\mathtt{M}}
\newcommand{\N}{\mathtt{N}}
\renewcommand{\L}{\mathtt{L}}
\renewcommand{\S}{\mathtt{S}}

\newcommand{\tydos}{\del}
\newcommand{\muu}{\#_{i}}
\newcommand{\mud}{\#_{e}}
\newcommand{\mudempty}{\#_{\mathtt{empty}}}
\newcommand{\mudu}{{\mathtt{bot}_{e}}_1}
\newcommand{\mudd}{{\mathtt{bot}_{e}}_2}
\newcommand{\gta}{A}

\newcommand{\ieml}{\L_{\emm}}% infinite list of empty multisets
\newcommand{\nom}{nom}

% added by Pierre

\newcommand{\rew}{\rightarrow}                  % !!! temporaire

% jugements gris
\newcommand{\lgray}[1]{\textcolor{gray}{#1}}
\newcommand{\lmuju}[3]{\lgray{#1\vdash} #2  \mid  #3} 
\newcommand{\lmuJu}[3]{\lgray{#1\Vdash} #2  \mid  #3}

% termes remarquables
\newcommand{\muagr}{\mu \al.\co{\gam}r}
\newcommand{\muagrs}{(\muagr)s}
\newcommand{\muagrsa}{\muagr \ire{\al}{s}}
\newcommand{\muac}{\mu \al.\Com}
\newcommand{\muacs}{(\muac)s}
\newcommand{\muacsa}{\muac\ire{\al}{s}}


\newcommand{\TypeV}{\mathcal{B}}               % set of type variables



\newcommand{\bgv}[1]{\bigvee\limits_{#1} }      % indexed type operations
\newcommand{\bgw}[1]{\bigwedge\limits_{#1}}
\newcommand{\suml}[1]{\sum\limits_{#1}}

\newcommand{\sigi}{\sigma_i}                   % indexed types etc
\newcommand{\sigk}{\sigma_k}                   % indexed types etc
\newcommand{\sigl}{\sigma_{\ell}}                   % indexed types etc
\newcommand{\sigj}{\sigma_j}                   % indexed types etc
\newcommand{\sigij}{\sigma_{i,j}}
\newcommand{\taul}{\tau_\ell}
\newcommand{\taui}{\tau_i}
\newcommand{\tauj}{\tau_j}
\newcommand{\gami}{\gamma_i}
\newcommand{\Gami}{\Gamma_i}
\newcommand{\Gaml}{\Gamma_{\ell}}
\newcommand{\Gamj}{\Gamma_j}
\newcommand{\Gamij}{\Gamma_{i,j}}
\newcommand{\Deli}{\Delta_i}
\newcommand{\Dell}{\Delta_{\ell}}

\newcommand{\Delij}{\Delta_{i,j}}
\newcommand{\Phiij}{\Phi_{i,j}}
\newcommand{\Phii}{\Phi_i}
\newcommand{\Phit}{\Phi_t}
\newcommand{\Phil}{\Phi_{\ell}}
\newcommand{\Phiul}{\Phi_u^{\ell}}
\newcommand{\Phiuk}{\Phi_u^{k}}
\newcommand{\Phikv}{\Phi_v^{k}}


\newcommand{\calC}{\mathcal{C}}




\newcommand{\length}{\mathtt{ar}}                    % type operator and measures
\newcommand{\mlg}{\mathtt{mlg}}
\newcommand{\coar}{\mathtt{coar}}
\newcommand{\Hd}{\mathtt{Hd}}
\newcommand{\Tl}{\mathtt{Tl}}
                 
\newcommand{\Ji}{J(i)}                  % indexation
\newcommand{\Jk}{J(k)}                  % indexation
\newcommand{\jJi}{j \in \Ji}                  % indexation
\newcommand{\jJk}{j \in \Jk}                  % indexation


\newcommand{\IM}{\mathcal{I}}
\newcommand{\IMi}{\mathcal{I}_i}
\newcommand{\IMl}{\mathcal{I}_{\ell}}
\newcommand{\IMj}{\mathcal{I}_j}
\newcommand{\IMu}{\IM_u}
\newcommand{\IMp}{\IM_p}
\newcommand{\UM}{\mathcal{U}}
\newcommand{\VM}{\mathcal{V}}
\newcommand{\VMC}{\mathcal{V}_{\Com}}
\newcommand{\VMCu}{\mathcal{V}_{\Com u}}
\newcommand{\VMu}{\mathcal{V}_{u}}
\newcommand{\VMal}{\VM_{\al}}
\newcommand{\VMalp}{\VM_{\al'}}

\newcommand{\UMi}{{\UM}_i}
\newcommand{\VMi}{{\VM}_i}
\newcommand{\VMj}{{\VM}_j}
\newcommand{\VMl}{{\VM}_{\ell}}

\newcommand{\UMij}{{\UM}_{i,j}}
\newcommand{\inter}{\wedge}
\newcommand{\union}{\vee}


\newcommand{\Com}{c}
\renewcommand{\bot}{\umult{\,}}


\newcommand{\Inde}[1]{{#1}(e)}
\newcommand{\Indne}[1]{{#1}(ne)}
\newcommand{\Ie}{\Inde{I}}
\newcommand{\Ine}{\Indne{I}}


\newcommand{\iIe}{i \in \Ie}
\newcommand{\iIne}{i \in \Ine}
\newcommand{\emul}{\mult{\, }} 
\newcommand{\eumul}{\umult{\,}}

\newcommand{\tGam}[1]{\Gam(#1)}
\newcommand{\tDel}[1]{\Del(#1)}


\renewcommand{\emph}[1]{{\it  #1}}
\newcommand{\subterm}{\triangleleft}

% macros créees pour remplacer les anciens indices et pour le lemme de subst







\newcommand{\tlL}[1]{\ell \in L(#1)}          % pas encore utilisée !
\newcommand{\pP}{p\in P}

\newcommand{\IMk}{\IM_k}      % types indicés
\newcommand{\UMj}{\UM_j}
\newcommand{\UMk}{\UM_k}
\newcommand{\UMkj}{\UM_{k,j}}
\newcommand{\VMk}{\VM_k}

\newcommand{\WM}{\mathcal{W}}
\newcommand{\WMl}{\WM_{\ell}}
\newcommand{\UMl}{\UM_{\ell}}
\newcommand{\uVMk}{\union_{\kK} \VMk}
\newcommand{\uIVMk}{ \umult{\IMk \rew \VMk}_{\kK}}

\newcommand{\IVMk}{\umult{\IMk \rew \VMk}_{\kK}} % macro a supprimer (redondante ac uIVMk)

\newcommand{\Gamk}{\Gam_k}            % environnements et preuves indicés
\newcommand{\Gamkj}{\Gam_{k,j}}
\newcommand{\Gamp}{\Gam_p}
\newcommand{\Gamstt}{\Gam_{\cxtt}}
\newcommand{\Gamscc}{\Gam_{\cxcc}}
\newcommand{\Delj}{\Del_j}
\newcommand{\Delk}{\Del_k}
\newcommand{\Delkj}{\Del_{k,j}}
\newcommand{\Delp}{\Del_p}
\newcommand{\Delstt}{\Del_{\cxtt}}
\newcommand{\Delscc}{\Del_{\cxcc}}
\newcommand{\Phij}{\Phi_j}
\newcommand{\Phik}{\Phi_k}
\newcommand{\Phikj}{\Phi_{k,j}}
\newcommand{\Phip}{\Phi_p}
\newcommand{\Psil}{\Psi_{\ell}}                 
\newcommand{\Psiku}{\Psi_{k}^u}                 
\newcommand{\Psiul}{\Psi^{\ell}_u}                 
\newcommand{\Theul}{\Theta^{\ell}_u}                 
\newcommand{\Theuu}{\Theta^1_u}                 
\newcommand{\Theud}{\Theta^2_u}                 
\newcommand{\Theu}{\Theta_u}                 
\newcommand{\Theuk}{\Theta^{k}_u}                 
\newcommand{\Phiku}{\Phi_{k}^u}                 
\newcommand{\Thetal}{\Theta_{\ell}}
\newcommand{\Xil}{\Xi_{\ell}}
\newcommand{\Xilu}{\Xi^{\ell}_u}
\newcommand{\Xiul}{\Xi^{\ell}_u}
\newcommand{\Xiuk}{\Xi^{\k}_u}

\newcommand{\TypCom}{\#}
\newcommand{\Typevide}{\umult{\mult{\,}\rew \umult{\,}}}
\newcommand{\cte}{\bullet}
\newcommand{\Empty}{\mathcal{E}}
\newcommand{\e}{{\it e}}

\newcommand{\AM}{\mathcal{A}}
\newcommand{\AMk}{\AM_k}
\newcommand{\AMl}{\AM_\ell}
\newcommand{\AMp}{\AM_p}
\newcommand{\arob}{\symbol{64}}
\newcommand{\muju}[3]{#1 \vdash #2  \mid  #3} 
\newcommand{\muJu}[3]{#1 \Vdash #2  \mid  #3} 
\newcommand{\UMp}{\UM_p}
\newcommand{\VMp}{\VM_p}
\newcommand{\Psip}{\Psi_p}
\newcommand{\Thetap}{\Theta_p}
\newcommand{\Xip}{\Xi_p}
\newcommand{\Psiq}{\Psi_q}
\newcommand{\Thetaq}{\Theta_q}
\newcommand{\Xiq}{\Xi_q}
\newcommand{\JM}{\mathcal{J}}
\newcommand{\JMk}{\mathcal{J}_k}
\newcommand{\JMl}{\JM_{\ell}}
\newcommand{\WMk}{\WM_k}
\newcommand{\ZM}{\mathcal{Z}}
\newcommand{\ZMl}{\ZM_{\ell}}
\newcommand{\WMq}{\WM_q}
\newcommand{\ET}[2]{ \mathtt{ET}(#1,\,#2)}

\newcommand{\Psik}{\Psi_k}
\newcommand{\many}{\inter}


\newcommand{\Q}{ \mathtt{Q} }
\newcommand{\Qo}{\Q_0}
\newcommand{\Qp}{\Q_p}
\newcommand{\qQ}{q\in \Q}
\newcommand{\qQo}{q\in \Qo}
\newcommand{\qQp}{q \in \Qp}

\newcommand{\calF}{\mathcal{F}}
\newcommand{\kKi}{{k\in K(i)}}
\newcommand{\FM}{ \mathcal{F} }
\newcommand{\GM}{ \mathcal{G} }
\newcommand{\calFi}{\calF_i}
\newcommand{\Delik}{\Del_{i,k}}
\newcommand{\IMik}{\IM_{i,k}}
\newcommand{\UMik}{\UM_{i,k}}
\newcommand{\uU}{\vee_{\iI} \UMi}
\newcommand{\uF}{\vee_{\iI} \calF_i}
\newcommand{\uUi}{\vee_{\kK} \UM_{\kK(i)}}
\newcommand{\secu}{^{\prime \prime}}

\newcommand{\Gamsec}{\Gam\secu}
\newcommand{\Delsec}{\Del\secu}

\newcommand{\Delo}{\Del_0}
\newcommand{\Delu}{\Del_u}
\newcommand{\Gamu}{\Gam_u}
\newcommand{\Gamo}{\Gam_0}
\newcommand{\Gamt}{\Gam_t}
\newcommand{\Delt}{\Del_t}
\newcommand{\Phio}{\Phi_0}
\newcommand{\UMo}{\UM_0}
\newcommand{\VMo}{\VM_0}
\newcommand{\FMo}{\FM_0}
\newcommand{\FMp}{\FM_p}
\newcommand{\GMo}{\GM_0}
\newcommand{\GMp}{\GM_p}
\newcommand{\ZMo}{\ZM_0}
\newcommand{\ZMp}{\ZM_p}
\newcommand{\Thetak}{\Theta_k}
\newcommand{\Xik}{\Xi_k}
\newcommand{\Lo}{\L_o}
\newcommand{\lLo}{\ell \in \Lo}
\newcommand{\lLp}{\ell \in \Lp}

\newcommand{\lo}{\ell_0}
\newcommand{\loL}{\ell_0 \in L}

\newcommand{\alu}{\ire{\al}{u}}
\newcommand{\alw}{\ire{\al}{w}}
\newcommand{\subxu}{\isubs{x/u}}

\newcommand{\K}{ \mathtt{K} }
\newcommand{\Ke}{\K(e)}
\newcommand{\Kne}{\K(ne)}       
\newcommand{\kKe}{j\in \Ke}     
\newcommand{\kKne}{j \in \Kne}  
\newcommand{\rempl}[3]{\langle #1 / \!\! / #2 . #3 \rangle} 
\newcommand{\ctx}{\mathtt{T}}
\newcommand{\ctxp}{\mathtt{T}'}
\newcommand{\otx}{\mathtt{C}}
\newcommand{\otxp}{\mathtt{C}'}
\newcommand{\gtx}{\mathtt{O}}
\newcommand{\gtxp}{\mathtt{O}'}


% nouveau set de commandes pour les contextes cx = 'context'
\newcommand{\cxtt}{\mathtt{TT}}
\newcommand{\cxtc}{\mathtt{TC}}
\newcommand{\cxct}{\mathtt{CT}}
\newcommand{\cxcc}{\mathtt{CC}}
\newcommand{\cxot}{\mathtt{OT}}
\newcommand{\cxoc}{\mathtt{OC}}

\newcommand{\cxterm}{\mathtt{T}}
\newcommand{\cxcommand}{\mathtt{C}}
\newcommand{\cxobject}{\mathtt{O}}


%\newcommand{\lmuex}{\lambda {\mu \mathtt{s}}}
\newcommand{\lmuex}{\lambda {\mu \mathtt{s}}}
\newcommand{\lmu}{\lambda {\mu}}
\newcommand{\nonelmuex}{\lambda {\overline{\mu\mathtt{r}}}}
\newcommand{\choice}[1]{#1^*}
\newcommand{\Any}{\mathcal{A}}
\newcommand{\ComTyp}{\mathcal{C}}
\newcommand{\lexnl}[1]{  \langle \eta(#1), |#1| \rangle  }


\newcommand{\mM}{m \in M}
\newcommand{\VMm}{\VM_m}
\newcommand{\UMm}{\UM_m}

\renewcommand{\vec}[1]{\overline{#1}}
\newcommand{\X}{\mathcal{X}}

\newcommand{\isz}[1]{\szm #1 }
\newcommand{\usz}[1]{\szm #1}
\newcommand{\szm}{\#}


\newcommand{\Phiu}{\Phi_u}
\newcommand{\Phiv}{\Phi_v}
\newcommand{\PhiCom}{\Phi_\Com}
\newcommand{\Gamv}{\Gam_v}
\newcommand{\GamCom}{\Gam_\Com}
\newcommand{\Delv}{\Del_v}
\newcommand{\DelCom}{\Del_\Com}
\newcommand{\IMt}{\IM_t}
\newcommand{\IMv}{\IM_v}

\newcommand{\Thetu}{\Theta^t_u}
\newcommand{\Thevu}{\Theta^v_u}
\newcommand{\Thealu}{\Theta^{\al}_u}
\newcommand{\Gamlv}{\Gam^{\ell}_v}
\newcommand{\Gamtu}{\Gam^t_u}
\newcommand{\Gamvu}{\Gam^v_u}
\newcommand{\Gamalu}{\Gam^{\al}_u}
\newcommand{\Gamuu}{\Gam^{1}_u}
\newcommand{\Gamud}{\Gam^{2}_u}

\newcommand{\Deluu}{\Del^{1}_u}
\newcommand{\Delud}{\Del^{2}_u}

\newcommand{\Deltu}{\Del^t_u}
\newcommand{\Delvu}{\Del^v_u}
\newcommand{\Delalu}{\Del^{\al}_u}
\newcommand{\Dellv}{\Del^{\ell}_v}
\newcommand{\IMlv}{\IM^{\ell}_v}
\newcommand{\orc}{\mathtt{OR}}
\newcommand{\andc}{\mathtt{AND}}
\newcommand{\Ua}{\mathcal{A}}
\newcommand{\Ub}{\mathcal{B}}
\newcommand{\Uy}{\UM_{y}}

\newcommand{\calH}{\mathcal{H}}
\newcommand{\calS}{\mathcal{S}}

\newcommand{\Hl}{\calH_\l}
\newcommand{\Sl}{\calS_\l}
\newcommand{\Hpl}{\calH'_\l}
\newcommand{\Spl}{\calS'_\l}
\newcommand{\Hlmu}{\mathcal{H}_{\lmu}}
\newcommand{\Slmu}{\mathcal{S}_{\lmu}}
\newcommand{\Slmuex}{\mathcal{S}_{\lmuex}}


\newcommand{\iIMsk}{\inter_{\kK} \choice{\IMk} }
\newcommand{\uVMkt}{\union_{\kK_t} \VMk}
\newcommand{\uVMkal}{\union_{\kK_{\al}} \VMk}
\newcommand{\uIVMkt}{\umult{\IMk \rew \VMk}_{\kK_t}}
\newcommand{\uIVMkal}{\umult{\IMk \rew \VMk}_{\kK_{\al}}}



%\newenvironment{proof}
%    {\begin{IEEEproof}
%    }
%    {
%    \end{IEEEproof}
%    }


\newcommand{\sset}{\mathcal{S}}

\newcommand{\phdot}{\phantom{.}}
\newcommand{\ftype}{\Rightarrow}
\newcommand{\Blind}{\xi }

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> strong-normalization.tex <==
\section{Strongly Normalizing $\lmu$-Objects}
\label{s:sn}



In this section we show the characterization of strongly-normalizing
terms of the $\l\mu$-calculus by means of the typing system introduced
in Section~\ref{s:types-lambda-mu}, \ie\ we show that an object $o$ is
strongly-normalizing iff $t$ is typable. \technicalreport{The proof of our main result
(Theorem~\ref{t:final}) relies  on the following three
ingredients:

\begin{itemize}
\item We define an inductive  set $\ISN{\lmu}$ which turns to be equivalent to the set of $\lmu$-strongly
normalizing objects $\SNSP$ (Lemma~\ref{l:caract}).
\item We show that every typable object is in $\ISN{\lmu}$ (Lemma~\ref{l:typable-isn}).  
\item We show that every $o$ in $\ISN{\lmu}$ is typable (Lemma~\ref{l:isn-typable}).  
\item We conclude using the previous points. 
\end{itemize}


We start by defining 
the inductive set $\ISN{\lmu}$ as  is the smallest subset of $\objects{\lmu}$ 
satisfying the following 
closure properties: 

\begin{enumerate}[\hspace*{0.3m}(1)]
\item  If $t_1 , \ldots  , t_n\ (n \geq 0) \in \ISN{\lmu}$, then $xt_1 \ldots t_n \in \ISN{\lmu}$. 
\item If  $t \in \ISN{\lmu}$, then $\l x.t \in \ISN{\lmu}$. 
\item If  $\Com  \in \ISN{\lmu}$, then $\mu \al.\Com \in \ISN{\lmu}$. 
\item If  $t \in \ISN{\lmu}$, then $\co{\al}t \in \ISN{\lmu}$.
\item If $u, t\isubs{x/u}\vec{v}\ (n \geq0) \in \ISN{\lmu}$, then $(\l x.t)u \vec{v} \in \ISN{\lmu}$. 
\item If $u, (\mu \al. \Com\ire{\al}{u})  \vec{v}\ (n \geq0)  \in \ISN{\lmu}$, then $(\mu \al.\Com)u \vec{v}\in \ISN{\lmu}$. 
\item If $u, (\mu \al. \Com\ire{\al}{u})  \vec{v}\ (n \geq0)  \in \ISN{\lmu}$, then $(\mu \al.\Com)u \vec{v}\in \ISN{\lmu}$. 
%\item If $\Com\isubs{\al/\beta}\in\ISN{\lmu}$, then $\co{\beta}\mu\al.\Com\in\ISN{\lmu}$. 
\end{enumerate}




We can formally relate $\SNSP$ and $\ISN{\lmu}$:  
\begin{lem}
\label{l:caract}
$\SNSP = \ISN{\lmu}$.
\end{lem} 

\begin{proof} $\SNSP \subseteq \ISN{\lmu}$ is proved by induction on
the pair $\lexnl{o}$ (both defined in Section~\ref{s:calculus}) using the  lexicographic order, while
$\ISN{\lmu} \subseteq \SNSP $ is proved by induction on 
$\ISN{\lmu}$ using Cor.~\ref{c:o-subs-sn-implique-o-sn}.
\end{proof} 
}




The proof of our main result (Theorem~\ref{t:final}) relies  on the following two ingredients:
\begin{itemize}  
\item Every $\Slmu$-typable object is in $\SN{\lmu}$ (Lemma~\ref{l:typable-isn}).  
\item Every object in $\SN{\lmu}$ is $\Slmu$-typable (Lemma~\ref{l:isn-typable}).  
%\item We conclude using the previous points. \\
\end{itemize}


First, we inductively reformulate the set of strongly normalizing objects:
the set $\ISN{\lmu}$ is defined as  the smallest subset of $\objects{\lmu}$  satisfying the following closure properties:
\begin{itemize}
\item[(1)]  If $t_1 , \ldots  , t_n\ (n \geq 0) \in \ISN{\lmu}$, then $x\, t_1 \ldots t_n \in \ISN{\lmu}$. 
\item[(2)] If  $t \in \ISN{\lmu}$, then $\l x.t \in \ISN{\lmu}$. 
\item[(3)] If  $\Com  \in \ISN{\lmu}$, then $\mu \al.\Com \in \ISN{\lmu}$. 
\item[(4)] If  $t \in \ISN{\lmu}$, then $\co{\al}t \in \ISN{\lmu}$.
\item[(5)] If $u, t\isubs{x/u}\vec{v}\ (n \geq0) \in \ISN{\lmu}$, then $(\l x.t)u \vec{v} \in \ISN{\lmu}$. 
 \item[(6)] If $u, (\mu \al. \Com\ire{\al}{u})  \vec{v}\ (n \geq 0)  \in \ISN{\lmu}$, then  $(\mu \al.\Com)u \vec{v}\in \ISN{\lmu}$.\\
\end{itemize}
  %\item If $\Com\isubs{\al/\beta}\in\ISN{\lmu}$, then $\co{\beta}\mu\al.\Com\in\ISN{\lmu}$.


\noindent The sets $\SN{\lmu}$ and $\ISN{\lmu}$ turn out to be equal, as expected:
\begin{lem}
\label{l:caract}
$\SN{\lmu}=\ISN{\lmu}$.
\end{lem} 
\begin{proof} $\SN{\lmu} \subseteq \ISN{\lmu}$ is proved by induction on
  the pair $\lexnl{o}$ endowed with the  lexicographic order,
  \modifrefb{where $\eta_{\lmuex}(o)$ is defined at the beginning of Section~\ref{s:calculus}}, and $|o|$ denotes the size of  $o$.
$\ISN{\lmu} \subseteq \SN{\lmu}$ is proved by induction on 
$\ISN{\lmu}$ using Cor.~\ref{c:o-subs-sn-implique-o-sn}.  
No reducibility argument is then needed in this proof.
\end{proof} 



\technicalreport{
As explained, we first show that any typable object $o$ belongs to $\SN{\lmu}$. }

\begin{lem} 
\label{l:typable-isn}
If  $o$ is $\Slmu$-typable,  then  $o  \in  \SN{\lmu}$. 
\end{lem}


%% short proof
%% \begin{proof}
%%   We show $o \in \ISN{\lmu} = \SN{\lmu}$ by induction on the size of
%%   typing derivations using Property~\ref{l:sr} for the non-erasing case,
%%   and building a new smaller type derivation in the erasing case.
%%   \end{proof}


\begin{proof} We proceed by induction on  $\sz{\Phi}$, where $\Phi   \tri\Gam \vdash  o:\Any \mid \Del$.  When $\Phi$ does not end
with the rule  $(\app)$ the proof is straightforward, 
so  we consider $\Phi$ ends with  $(\app)$, where  $\Any = \UM$ and $o  = xt_1 \ldots t_n$ or
$o = (\mu \al. \Com)t_1 \ldots t_n$ or 
$o  = (\l x.  u)t_1 \ldots t_n$, where $n \geq 1$. \\
By construction  there are subderivations
$(\Phi_{t_i})_{i \in \cset{1 \ldots n}}$
such that  $(\sz{\Phi_{t_i}} < \sz{\Phi})_{i \in \cset{1 \ldots n}}$ so that
the \ih\ gives 
 $(t_i \in \ISN{\lmu})_{i \in \cset{1 \ldots n}}$. There are three different cases: \\
If $o=xt_1 \ldots t_n$, then from $t_i \in \ISN{\lmu}\ (1 \leq i \leq n)$
we conclude directly $x t_1 \ldots t_n \in \ISN{\lmu}$. \\
If $o = (\mu \al. \Com)t_1 \ldots t_n$, there are two cases: 
\begin{itemize}
 \item $\al \in \fn{\Com}$.  Using  Property~\ref{l:sr} we get  $\Phi' \tri
   \tyj{(\mu \al. \Com\ire{\al}{t_1}) t_2 \ldots t_n }{\Gam}{\UM \mid
     \Del}$ and $\sz{\Phi'} < \sz{\Phi}$. Then the \ih\ gives $(\mu
   \al. \Com\ire{\al}{t_1}) t_2 \ldots t_n \in \ISN{\lmu}$. This,
   together with $t_1 \in \ISN{\lmu}$ gives $o  \in
   \ISN{\lmu}$.
 \item $\al  \notin \fn{\Com}$. 
 Then it is easy to build a  type derivation
 $\Phi'  \tri \tyj{(\mu \al. \Com) t_2 \ldots t_n}{\Gam'}{\UM  \mid \Del'}$ verifying
 $\sz{\Phi'} < \sz{\Phi}$, so that $(\mu \al. \Com) t_2 \ldots t_n \in \ISN{\lmu}$ holds by the \ih\ 
 This, together with with $t_1 \in \ISN{\lmu}$ gives 
             $o  \in \ISN{\lmu}$. 
 \end{itemize}
If $o=(\l x. u)t_1 \ldots t_n$, we reason similarly to the previous one.
%%  \begin{itemize}
%%  \item $x \in \fv{u}$. 
%%  Using Property~\ref{l:sr} we get $\Phi' \tri  \tyj{u\isubs{x/t_1}t_2 \ldots t_n}{\Gam }{\UM \mid  \Del}$ such that 
%%              $\sz{\Phi'} < \sz{\Phi}$. Then the \ih\ gives 
%%              $u\isubs{x/t_1}t_2 \ldots t_n \in \ISN{\lmu}$. 
%%   This, together with $t_1 \in \ISN{\lmu}$ gives  
%%   $o \in \ISN{\lmu}$.
%% \item $x \notin \fv{u}$.
%%   Then it is easy to build a type derivation
%%   $\Phi'  \tri \tyj{u t_2 \ldots t_n}{\Gam'}{\UM  \mid \Del'}$ verifying
%% $\sz{\Phi'} < \sz{\Phi}$, so that $u t_2 \ldots t_n \in \ISN{\lmu}$ holds by the \ih\ 
%% This, together with with $t_1 \in \ISN{\lmu}$ gives 
%%             $o  \in \ISN{\lmu}$. 
%%  \end{itemize}
  \end{proof}


Normalization also implies typability:


\begin{lem}
\label{l:isn-typable}
If $o \in \SN{\lmu}$, then  $o$ is $\Slmu$-typable. 
\end{lem}

\begin{proof}
Thanks to Lemma~\ref{l:caract}, we can reason by induction on  
$o \in \ISN{\lmu}=\SN{\lmu}$.  The four first cases
are straightforward.

Let $o = (\l x. u)v t_1 \ldots t_n \in \ISN{\lmu}$ coming from
$u\isubs{x/v} t_1 \ldots t_n, v  \in \ISN{\lmu}$. By the \ih\ 
$u\isubs{x/v} t_1 \ldots t_n$ and $v$ are both typable. We consider two cases.
If $x \in \fv{u}$, then $(\l x. u)v t_1 \ldots t_n$ is typable
by \modifref{Property~\ref{l:se-s}}. Otherwise, by construction, we get
typing derivations for $u, t_1 \ldots, t_n$ which can easily be used  to 
build a typing derivation of $(\l x. u)v t_1 \ldots t_n$. 

Let $o = (\mu \al. \Com)v t_1 \ldots t_n \in \ISN{\lmu}$ coming from 
$(\mu \al. \Com\ire{\al}{v}) t_1 \ldots t_n, v  \in \ISN{\lmu}$. By the \ih\ 
$(\mu \al. \Com\ire{\al}{v}) t_1 \ldots t_n$ and $v$ are both typable. We consider two cases.
If $\al  \in \fn{\Com}$, then $(\mu \al. \Com)v t_1 \ldots t_n$ is typable
by \modifref{Property~\ref{l:se-s}}. Otherwise, by construction, we get
typing derivations for $\Com, t_1 \ldots, t_n$ which can easily be used  to 
build a typing derivation of $(\mu \al. \Com)v t_1 \ldots t_n $. 
\end{proof} 

Lemmas~\ref{l:typable-isn} and~\ref{l:isn-typable}  allow us to conclude 
with the main result of this paper which is  the equivalence between typability and 
strong-normalization for the $\lmu$-calculus.  Notice that no 
reducibility argument was used in the  whole proof. 

\begin{thm}
  \label{t:final}
Let $o \in \objects{\lmu}$. Then $o$ is typable in system $\Slmu$ iff
$o \in \SN{\lmu}$.  Moreover, if $o$ is $\Slmu$-typable with tree
derivation $\Pi$, then $\sz{\Pi}$  gives an upper bound to the maximal
length of a reduction sequence starting at $o$. 
\end{thm}



\modifref{ To prove the second part of the statement, \ie\ that
  $\sz{\Pi}$ bounds the length of every reduction sequence starting at
  $o$, it is sufficient to endow the system with \emph{non-relevant}
  axioms for variables and names, \ie\ to replace the rule $(\ax)$
  with the following weakened form:
$$
\infer{\UM \neq \eumul}{\muju{\Gam \inter x:\mult{\UM}}{x:\UM}{\Del}}\ (\mathtt{axw})  
$$ This extension of system $\Slmu$, called $\Slmu'$,  which does not satisfy subject expansion, is however sufficient to guarantee
\textit{weighted} subject reduction for erasing as well as for
non-erasing steps. The definition of $\sz{\_}$ in this new extended system
counts an $(\axw)$-rule for 1.  Thus, if $o$ is $\Slmu$-typable, let say by means of a typing derivation $\Pi$, then $o$ is also typable by means of the same derivation $\Pi$, with the same size $\sz{\Pi}$,  in the
extended system $\Slmu'$, and this is
  because rule $(\mathtt{axw})$ subsumes $(\ax)$.  By \textit{weighted} subject reduction in system
  $\Slmu'$, $\sz{\Pi}$ gives the expected upper bound.
  }




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> tools-for-sn.tex <==

\newpage

\section{\pierre{New appendix}}

\pierre{pas d'inspiration pour les titres, je les mets après}

\subsection{Orders on types and derivations}

The order $\leqty$, defined both on types and on derivation, materializes a loss of information.
Order on types.

$$
\begin{array}{ccc}
  \infer{}{a \leqty a} &  \infer{}{\TypCom \leqty \TypCom} & \infer{\IM \leqty \IM'\sep \tau \leqty \tau'}{\IM \rew \tau \leqty \IM' \rew \tau'}\\ \\
  \infer{  K \subeq K'\sep (\tau_k \leqty \tau'_k) }{\umult{\tau_k}_{\kK} \leqty \umult{\tau'_k}_{\kK'}} &
 &   
  \infer{  K \subeq K'\sep (\UM_k \leqty \UM'_k)_{\kK} }{
\mult{\UMk}_{\kK}\leqty \mult{\UM'_k}_{\kK'}}
\end{array}
$$
We also set $\Gam\leqty \Gam'$ if $\Gam(x)\leqty \Gam'(x)$ for all variables $x$ and $\Del\leqty \Del'$ if $\Del(\al)\leqty \Del'(\al)$ for all names $\al$.

\pierre{blah. insérer exemples}


Orders on derivations.
\begin{itemize}
\item $ \infer[(\ax)]{}{\muju{x:\mult{\UM}}{x:\UM}{\es}}\leqty \infer[(\ax)]{}{\muju{x:\mult{\UM'}}{x:\UM'}{\es}}$ when $\UM \leqty \UM'$.\\[0.2cm]
\item $\infer[(\mud)]{\Phi_c\tri\muju{\Gam}{c:\TypCom}{\Del,\al:\UM}}{\muju{\Gam}{\mu.c:\choice{\UM}}{\Del}}\leqty  \infer[(\mud)]{\Phi'_c\tri\muju{\Gam'}{c:\TypCom}{\Del',\al:\UM'}}{\muju{\Gam'}{\mu.c:\choice{(\UM')}}{\Del'}}$\\[0.2cm]
  \hfills when $\Phi_c\leqty \Phi'_c$ and $\choice{\UM}\leqty \choice{(\UM')}$ (this latter condition is necessary only when $\UM=\es$).\\[0.2cm]
\item $\infer[(\many)]{(\Phi'_k\tri t:\UM_k)_{\kK}}{t:\mult{\UM_k}_{\kK}} \leqty \infer[(\many)]{(\Phi'_k\tri t:\UM'_k)}{t:\mult{\UM_k}_{\kK'}}$
when  $K\subeq K'$ and $\Phi_k\leqty \Phi'_k$ for all $\kK$.\\[0.2cm]
\item $\infer[(\app)]{\Phi \tri t\sep \Theta\tri u}{t\,u}\leqty \infer[(\app)]{\Phi' \tri t'\sep \Theta'\tri u'}{t'\,u'}$ when $\Phi\leqty \Phi'$, $\Theta\leqty \Theta'$.
  \\[0.2cm]
  
\end{itemize}
By induction, one checks that, if $\Phi\tri \muju{\Gam}{o:\Any}{\Del}$, $\Phi'\tri \muju{\Gam'}{o':\Any'}{\Del'}$, then $o=o'$, $\Gam\leqty \Gam'$, $\Any \leqty \Any'$ and $\Del\leqty \Del'$




\subsection{Typing multiplicity and cumulated arity}

The support of an object: $\supp{x}=\myset{\epsi}$, $\supp{\coal t}=\supp{\lx.t}=\sepsi \cup 0 \ct \supp{t}$, $\supp{\mu.c}=\sepsi \cup 0\ct \supp{c}$, $\supp{t\,u}=\sepsi \cup 1\ct \supp{t} \cup 2 \ct \supp{u}$.\\


The set of positions of a variable $x$ in $t$:
\begin{itemize}
\item $\posx{\Pi}=1$ when $t=x$.
\item $\posx{\Pi}=0$ when $t=\lx.t_0$.  
\item $\posx{\Pi}=0\ct \posx{\Pi_0}$, in the other cases when the conclusion of $\Pi$ has only one premise and $\Pi_0$ is the immediate subderivation of $\Pi$.
\item \pierre{app}
\item \pierre{many}
\end{itemize}


\pierre{idem with names}\\

$\mulbPi$: the number of times the position $b\in \supp{t}$ is typed in $\Pi\tri t$.

\pierre{pourquoi en a-t-on besoin? Pour s'assurer que même en cas de réduction du sujet light (pas effacant), le réduit est moins typé}

\begin{itemize}
\item $\mulbPi=1$ if $b=\epsi$ and $\Pi$ is a regular derivation.
\item $\mulp{0\ct b}{Pi}=\mulb{\Pi_0}$, if the conclusion has only one premise, which is proved by subderivation $\Pi_0$.
\item $\mulp{1\ct b}{\Pi}=\mulb{\Pi_0}$ and $\mulp{2\ct b}{\Pi}=\mulb{\Theta}$ if $\Pi$ concludes with an $\app$-rule, $\Pi$ is the (regular) left  subderivation of $\Pi$ and $\Theta$ the (auxiliary) left subderivation.\\
\end{itemize}

If $B\subeq \supp{t}$, we set $\mulB{\Pi}=+_{\bB} \mulb{\Pi}$.\\


\pierre{Idem with the cumutated cardinality of names in a derivation.\\ }

\pierre{Définir résiduation ? ou pointeur vers la définition?}
si $b_* \in \supp{o}$ et $o$ admet un redex a la position $b$, alors $\Resb{b_*}$ denote l'ensemble des residus de la position $b_*$ quand réduit dans $o$ le redex a la position $b$.


\textbf{Lemma subst:} Idem + if $b\in o$, then $\mulb{\Phi_{o\subxu}}$ + if $b\in \supp{u}$, then $\mulp{\pos{x}{\Phi_o}\ct b }=\mulp{b}{\Theta_u}$\\
Remark: $|\IM|=\mulp{\pos{x}{\Phi_o}}$: \textbf{ceci nous permet de decrire la diminution en cardinalite dans la preuve de SR} \\

\textbf{Lemma repl.:} nouvelle clause\\



\textbf{Lemma s.r.:} If $\Phi \tri \muju{\Gam}{o:\Any}{\Del}$ and $o\rew_b o'$, then there is $\Phi'\tri \muju{\Gam'}{o':\Any'}{\Del'}$ such that $\sz{\Phi'}<\sz{\Phi}$ and:
\begin{itemize}
\item for all $b_*\in \supp{t}$, $\mulp{\Resb(b_*)}{\Phi'}\leqs  \mulp{b_*}{\Phi}$.

\item idem avec cumulated arity.
\end{itemize}



\begin{proof}
  Induction on $\sz{\Phi}$, using both the substitution and the antisubstitution lemma to capture this kind of steps (on s'interesse a la reduction de la premire ligne):\\

$\begin{array}{ccc}
(\lx.r)s\,t_1\ldots t_q &  ?  & (\lx.r)s'\,t_1\ldots t_q \\
\downarrow &  & \downarrow \\
r\isubs{x/s}\,t_1\ldots t_q & \rew^* & r\isubs{x/s'}\,t_1\ldots t_q    
\end{array}$\\

  Comment procede-t-on ?
  \begin{itemize}
    \item Si $x$ occure dans $r$, on utilise le lemme de subsitution pour typer $t_0=r\isubs{x/s}$ avec une plus petite dérivation. Donc l'i.h. s'applique sur $t_0$. On obtient donc une dérivation $\Pi'_0$ typant $t'_0=r\isubs{x/s'}\,t_1\ldots t_q$. On utilise alors le lemme d'\textbf{***anti-substitution***} sur $\Pi'_0$ pour obtenir une dérivation $\Pi'$ typant $(\lx.r)s'\,t_1\ldots t_q$. On a bien $\sz{\Pi'}<\sz{\Pi}$, parce qu'on sait que $s'$ n'est pas typé plus de fois dans $t'_0$ que dans $t_0$ (c'est la le \textbf{point crucial} et chiant, qui fait qu'on doit renforcer nos hypotheses d'induction).
    \item Pas compliqué, repose aussi sur l'i.h. concernant les multiplicités.
    \item Grace au theoreme des dvp complets, on peut traiter les cas ou on reduit dans $r$, $s$ ou l'un des $t_i$ sans faire de distinction.
  \end{itemize}
Note que de cette facon, on n'a pas besoin de faire la reformulation de SN en ISN.   
\end{proof}




%\begin{array}{c}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

